Dynamic Mobile Manipulation via Whole-Body Bilateral Teleoperation of a Wheeled Humanoid

Humanoid robots have the potential to help human workers by realizing physically demanding manipulation tasks such as moving large boxes within warehouses. We define such tasks as Dynamic Mobile Manipulation (DMM). This paper presents a framework for DMM via whole-body teleoperation, built upon three key contributions: Firstly, a teleoperation framework employing a Human Machine Interface (HMI) and a bi-wheeled humanoid, SATYRR, is proposed. Secondly, the study introduces a dynamic locomotion mapping, utilizing human-robot reduced order models, and a kinematic retargeting strategy for manipulation tasks. Additionally, the paper discusses the role of whole-body haptic feedback for wheeled humanoid control. Finally, the system's effectiveness and mappings for DMM are validated through locomanipulation experiments and heavy box pushing tasks. Here we show two forms of DMM: grasping a target moving at an average speed of 0.4 m/s, and pushing boxes weighing up to 105\% of the robot's weight. By simultaneously adjusting their pitch and using their arms, the pilot adjusts the robot pose to apply larger contact forces and move a heavy box at a constant velocity of 0.2 m/s.

==> DynamicSimilarity.tex <==
\section{Dynamically Similiar Locomotion Retargeting}
In this work, the telelocomotion mapping models the human and robot as pendulum systems to generate dynamically consistent references for tracking. The use of human haptic feedback enables the use of virtual springs and force feedback to give the pilot a larger range of motion and information about the robot's external interaction forces as a step towards human-robot immersion. \marty{Tie mapping and bilateral telop together better. In other words, the paper is a teleoperation paper more than a pure mapping paper. Tie together desire for haptics in teleoperation to why the mapping was made this way}

%Under the proposed bilateral teleoperation framework,

Section \ref{subsec:HumanModel} motivates the human fixed-based actuated inverted pendulum (AIP) model. Section \ref{subsec:RobotModel} derives a condition for stabilizing the robot cart-pole given by its unitless DCM. Section \ref{subsec:DynSim} shows the dynamically similar locomotion mapping and defines the haptic feedback law.
% We note that the upper body movements are treated as unmodeled disturbances.


\subsection{Human Motion Model} \label{subsec:HumanModel}

% Classically the LIP has been used to abstract human bipedal locomotion \cite{???}. The LIP pitch angle is traditionally computed between the CoP and CoM, and converges to zero in steady state as the CoP tracks the CoM. 
Use of human pitch for hands-free teleoperation and control of wheeled humanoids has shown viability \cite{Puru2022}. Attempting to capture the pitch angle from classically used human locomotion models, such as the LIP, presents a problem however. This  angle - defined between the human CoP and CoM - converges to zero in steady state as the CoP tracks the CoM.
This results in stop-and-go motions and unintuitive pitch control on wheeled robots. For example, the human may lean at a constant angle, but the desired reference is zero causing the robot be upright.

% This results in stop-and-go motions on wheeled robots tracking desired pitch trajectories. 
%as the CoP tracks the CoM. 

Thus, we propose applying a slight transformation to model the human as a fixed-base actuated inverted pendulum (\textbf{AIP}) as shown in Fig. \ref{fig:Human-Robot Actuated Pendulum}. This in turn allows us to define the pitch angle between the fixed human ankle and their CoM. This measurement remains constant in steady state and does not change as a function of the CoP. Instead, the CoP is used to define the ankle torque needed to stabilize the human inverted pendulum. 

% The ankle height is given by $h_{aH}$ and is significantly smaller compared to the height of the center of mass, $h_H$. The human ankle torque $\tau_H$ and human pitch angle $\theta_{aH}$ are defined in the positive clockwise direction. The external force, $F_{HMI}$, is applied to the human CoM through a human machine interface \cite{wang2021dynamic}. 

The dynamics for the AIP are given by:
\begin{equation}
   \Ddot{\theta}_{H}=\frac{g}{h_H-h_{aH}}s_{\theta_{H}}+\frac{\tau_{H}}{m(h_H-h_{aH})^2}+\frac{F_{HMI}}{m(h_H-h_{aH})}c_{\theta_{H}}
\end{equation}
where $h_{aH}$ is the ankle height and $h_H$ is the CoM height. The human pitch angle, $\theta_{H}$, and human ankle torque, $\tau_H = p_{H}m_H g $, are defined in the positive clockwise direction. The external force, $F_{HMI}$, is applied to the human CoM through a human machine interface \cite{wang2021dynamic}.

Linearizing around the 0 upright position, and assuming $h_{H}>>h_{aH}$ allows us to write in State Space form:
% \begin{equation}
%    \Ddot{\theta}_{H}=\frac{g}{h_H}\theta_{H}+\frac{\tau_{H}}{mh_H^2}+\frac{F_{HMI}}{mh_H}
%    \label{eq:EOM_Human}
% \end{equation}
%\begin{equation}
%    m_H h_H^2 \Ddot{\theta} - m_H g h_H sin(\theta_H) = \tau_H 
%\end{equation}
% The state-space representation of (\ref{eq:EOM_Human}) is:
\begin{equation}
    \begin{bmatrix}
        \dot{\theta}_{H}\\ \ddot{\theta}_{H}
    \end{bmatrix} = 
    \begin{bmatrix}
        0 & 1\\
        \omega_{H}^2 & 0
    \end{bmatrix}
    \begin{bmatrix}
        \theta\\ \dot{\theta}
    \end{bmatrix} +
    \begin{bmatrix}
        0 \\
        \frac{1}{mh^{2}_{H}}
    \end{bmatrix} \tau_{H}
     +
    \begin{bmatrix}
        0 \\
        \frac{1}{mh_{H}}
    \end{bmatrix} F_{HMI}
\end{equation}
The state transition matrix has eigenvalues $\pm \omega_H$. Applying a changes of variables and writing in canonical form:
% and substituting for the human's stabilizing input actuation $\tau_H = p_{H}m_H g $:

\begin{equation} \label{eq:human_dcm}
    \begin{bmatrix}
        \dot{\zeta}_H\\ \dot{\xi}_H
    \end{bmatrix} = 
    \begin{bmatrix}
        -\omega_H & 0\\
        0 & \omega_H
    \end{bmatrix}
    \begin{bmatrix}
        \zeta_H\\ \xi_H
    \end{bmatrix} +
    \begin{bmatrix}
        \frac{1}{???} \\
        -\frac{1}{????}
    \end{bmatrix} p_H
\end{equation}

\marty{Highlight briefly the reason the DCM is the state we chose to track. Really its a design choice}
\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{Figures/HumanRobotTemplateModelsOverlay.pdf}
    \caption{\textbf{(A)} The proposed human actuated pendulum models the ankle as an actuator to control the lean of this non-minimum phase system - much like other pendulum systems. \textbf{(B)} The cart-pole model used for planning dynamically similar desired trajectory}
    \label{fig:Human-Robot Actuated Pendulum}
\end{figure}
% While linear inverted pendulums are often used as template model for bipedal locomotion, they may not represent the ideal model for control of wheeled robots. 
\subsection{Robot Cart-Pole DCM} \label{subsec:RobotModel}
% \yeongtae{I think it is better to include this subsection in the system overview section. We need to refer the robot figure for the exact notations such as the angle, direction, etc. Also, justification about why the cart pole model is introduced instead of WPI is necessary. I think we can introduce WPI instead of cart-pole, and use a symbol for the complex constants in A matrix. And describe it as "The humand and robot dynamics are similar, and this constant corresponds to the natural frequency term in human natural frequency."}
 % To the best of the authors' knowledge, the unitless DCM has not previously been studied for tracking and stabilization for this class of systems. 
We aim to stabilize the cart-pole system by tracking the human DCM as shown in Eq. \ref{eq:human_dcm}. As such, the unitless DCM for the linearized  cart-pole system is derived. \marty{The dcm is the unstable part of the dynamics that needs to be stabilized. Is that a good motivation?}

The cart-pole eigenvalues around its fixed point are given by:
\begin{equation}
    \begin{gathered}[b]
        \lambda_{x_w,\dot{x}_w} = 0 \\
        \lambda_{\theta_R,\dot{\theta}_R} = \pm \sqrt{\frac{g}{h_R}}
    \end{gathered}
\end{equation}
The states corresponding to eigenvalues at 0 indicate marginally stable behavior in these modes. In other words, these states neither grow nor decay when perturbed. To design control references that can stabilize the unstable dynamics we focus on isolating the non-zero eigenvalue variables $\theta_R$ and $\dot{\theta}_R$ :
\begin{equation} \label{dyn_of_int}
    \begin{bmatrix}
        \dot{\theta}_R\\ \ddot{\theta}_R
    \end{bmatrix} = 
    \begin{bmatrix}
        0 & 1\\
        \alpha\omega_R^2 & 0
    \end{bmatrix}
    \begin{bmatrix}
        \theta_R\\ \dot{\theta}_R
    \end{bmatrix} +
    \begin{bmatrix}
        0 \\
        \frac{-1}{Mh_R}
    \end{bmatrix} F_R
\end{equation}
where $\omega_R = \sqrt{\frac{g}{h_R}}$ is the linear natural frequency and $\alpha = \frac{m}{M}$ is a unitless quantity from Eq. \ref{linStateSpaceModel}.

Diagonlizing our state transition matrix, isolates the convergent, $\zeta_R$, and divergent components of motion, $\xi_R$, for the cart-pole system:

\begin{equation} \label{DCM_Def}
    \begin{bmatrix}
        \zeta_R \\ \xi_R
    \end{bmatrix} 
    =
    \begin{bmatrix}
        \theta_R - \frac{\dot{\theta}_R}{\alpha^{1/2}\omega_R}\\
        \theta_R + \frac{\dot{\theta}_R}{\alpha^{1/2}\omega_R}
    \end{bmatrix}
\end{equation}
letting $\omega_R^{'} = \alpha^{\frac{1}{2}}\omega_R$, the dynamics of interest can then be rewritten as such:
 
\begin{equation}
    \begin{bmatrix}
        \dot{\zeta}_R\\ \dot{\xi}_R
    \end{bmatrix} = 
    \begin{bmatrix}
        -\omega^{'}_R & 0\\
        0 & \omega^{'}_R
    \end{bmatrix}
    \begin{bmatrix}
        \zeta_R\\ \xi_R
    \end{bmatrix} +
    \begin{bmatrix}
        \frac{1}{\omega_R^{'} Mh_R} \\
        -\frac{1}{\omega_R^{'} Mh_R}
    \end{bmatrix} F_R
\end{equation}
\marty{To keep or not to keep. Come back to. Should discuss that theres no position or velocity tracking}We note that $\alpha$ is a ratio of the CoM mass to the robot wheel mass and can be viewed as effectively increasing the natural frequency of the system $\omega_R^{'} > \omega_R$ when $m >> M$ as $\alpha^{\frac{1}{2}} > 1$. Since the majority of mass is concentrated at the pole, and the base is much lighter we can move the cart underneath very quickly, effectively changing the robot lean angle. This can help the pilot in controlling dynamic stop and go motions of the robot. 


\subsection{Dynamically Similar Locomotion Mapping}\label{subsec:DynSim}

\begin{figure*}[t] 
    \centerline{\includegraphics[width=18.5cm]{Figures/SystemBlockDiagram.pdf}}
    \caption{(A) Full system layout and control flow work from pilot to the WIP to the full robot. (B) Overview of the control architecture. \marty{I need to add a signal for the camera feed back to human. Also fix labeling convention for left, right and human}}
    \label{figHMI}
    \vspace{-1.25em}
\end{figure*}
The proposed model-based mapping for humanoid tele-locomotion towards DMM accounts for the different sizes of the robot and human by normalizing along their natural frequency, masses, and heights \cite{ProfPaper2}.
By equating the human and robot’s angular dynamics, through their unitless DCM’s we can: 
\begin{itemize}
\item Generate references for robot tracking that utilize the human's strategy for dynamically pitching and stabilizing their body
\item Capture the non-minimum phase behavior of the human CoP as a feedforward for increased responsiveness  
\item Explicitly model and map virtual and external forces acting on the human and robot
\end{itemize}
We start by enforcing:
\begin{equation} \label{dcm_kin_sim}
    \begin{gathered}[b]
        \xi_R = \xi_H  \\
    \end{gathered}
\end{equation}
To satisfy this kinematic constraint on the motion of the two systems a dynamic constraint is imposed by taking the time derivative and normalizing by time:

\begin{equation} \label{Dyn_constraint}
    \begin{gathered}[b]
        \frac{\dot{\xi}_R}{\omega_R^{'}} = \frac{\dot{\xi}_H}{\omega_H}   \\
    \end{gathered}
\end{equation}
 where $\dot{\xi}_R = \dot{\theta}_R + \frac{\ddot{\theta}_R}{\omega_R^{'}}$ and $\dot{\xi}_H = \dot{\theta}_H + \frac{\ddot{\theta}_H}{\omega_H}$ are found by taking the time derivative of the DCM given by Eq. \ref{DCM_Def} and Eq. ??.

Expanding Eq. \ref{Dyn_constraint} by substituting for robot and human angular accelerations, Eq. \ref{eq:EOM_Human} and Eq.\ref{dyn_of_int}, we find the following relationship relating the pendular accelerations of the 2 systems:
\begin{equation} \label{eq:exp_dyn_sim}
        \theta_R \!+\! \frac{\dot{\theta}_R } {\omega_R^{'}} \!+\! \frac{(\frac{1}{\alpha})\hat{F}_{ext} - F_R}{m_R\omega_R^2 h_R} = 
        \theta_H \!+\! \frac{\dot{\theta}_H }{\omega_H} \!-\! \frac{p_H}{h_H} \!+\! \frac{F_{HMI}}{m_H\omega_H^2 h_H} 
\end{equation}

We choose a feedforward $F_R$ and feedback term $F_{HMI}$ accordingly:
\begin{equation}\label{eq:dyn_fb}
    \begin{gathered}
        F_R = m_R\omega_R^2 h_R \left(\frac{p_H}{h_H}\right) \\
        F_{HMI} \!=\! m_H\omega_H^2 h_H \! \left(\!\!(\theta_R \!-\! \theta_H) \!+\! \!\left(\frac{\dot{\theta}_R}{\omega^{'}_R} \!-\! \frac{\dot{\theta}_H}{\omega_H}\!\!\right)\!\!\right) \!+\!k_{c}\hat{F}_{ext} \\
        k_{c} = \frac{m_H\omega_H^2 h_H}{\alpha\; m_R \omega_R^2 h_R}
    \end{gathered}
\end{equation}
The feedback force effectively tries to push the human and robot together. The feedback here allows the human to understand the direction of the robots movement and plan their motion accordingly. The feedback sensation can be best represented as a ghost of the robot. The feedforward term captures the non-minimum phase dynamics of the CoP and is useful as a feedforward term as wheeled robots also are non-minimum phase systems. 

==> ManipulationMap.tex <==
\section{Kinematically Similar Manipulation Retargeting}
% \section{Mapping Methods for Whole Body DMM}

In this section we present the upper body motion retargeting strategy for manipulation. We leverage the similarity in joint topology of the human and robot arms to develop a kinematic mapping. We approximate robot and human shoulders as spherical wrists to simplify the inverse kinematics problem.
 
\subsection{Upper-body Arm Mapping}
 The vector of all arm joint angles is given by $q_a \in \R^{n_a\times2}$ where $n_a = 4$. The respective human and robot upper body generalized coordinates are given by:
\begin{equation}
    \begin{gathered}
        q^H_a = 
        \begin{bmatrix}
            {}_{r}q^H \\
            {}_{l}q^H
        \end{bmatrix}
        \;,\;\; 
        q^R_a = 
        \begin{bmatrix}
            {}_rq^R \\
            {}_lq^R
        \end{bmatrix}
        \\
        {}_iq^H = [q_0^H \; q_1^H \; q_2^H \; q_3^H]^T  \;,\;\; 
        {}_iq^R = [q_0^R \; q_1^R \; q_2^R \; q_3^R]^T 
    \end{gathered}
\end{equation}
where $i \in \{r,l\}$ represent the right and left arms. The pilot's motion and elbow position can be found through the forward kinematics of the motion capture suit. Thus, the unit vector from the human shoulder to the elbow can be defined as ${}_i\mathcal{R}^z_{H}$ as shown in Fig. \ref{fig:arm_retargeting} (A). For shorthand notation the subscript denoting the arm is not included in the derivations below. However, the computation is performed for both arms.

We note that the human elbow and robot elbow approximately move on spheres centered around their respective shoulders. Leveraging this similarity we choose the unit vector from the robot's shoulder to its elbow to be in the same direction as the humans, as seen in Fig. \ref{fig:arm_retargeting} (B):
\begin{equation}
    \mathcal{R}^z_{R} = \mathcal{R}^z_{H}
\end{equation}
To find the remaining axis we define the set of vectors, $\mathcal{S}$, perpendicular to $\mathcal{R}^z_H$:
\begin{equation}
    \mathcal{S} = \{\mathcal{R}_u \;|\; \mathcal{R}_u \cdot \mathcal{R}^z_H = 0\} 
\end{equation}
The second axis of rotation can be subsequently set:

\begin{equation}
    \mathcal{R}^y_R = \text{proj}_{\mathcal{S}}(\mathcal{R}^y_H)
\end{equation}
The aim of this projection is to find the vector closest to that of the human $\mathcal{R}^y_H$ that is also perpendicular to the given $\mathcal{R}^z_H$ as shown in Fig. \ref{fig:arm_retargeting} (B). The final axis is given by their cross product: $\mathcal{R}^x_R = \mathcal{R}^y_R \times \mathcal{R}^z_R$. With all 3 axis of the spherical wrist defined, constructing our rotation matrix, we can solve the inverse kinematics of the spherical wrist \cite{2021SphericalWrist} in the specified convention to find our desired robot arm joint angles:
\begin{equation}
    \begin{gathered}
        \left[\mathcal{R}^x_R \; ; \; \mathcal{R}^y_R \; ; \; \mathcal{R}^z_R \right] = 
        \begin{bmatrix}
            r_{11} & r_{12} & r_{13} \\
            r_{21} & r_{22} & r_{23} \\
            r_{31} & r_{32} & r_{33}
        \end{bmatrix}
        \\
        q^R_0 = \text{tan}^{-1}\left( \frac{r_{23}}{r_{13}}\right) \\ 
        q^R_1 = \text{tan}^{-1} \left(\frac{\sqrt{1 - r_{33}^2}}{r_{33}} \right) \\
        q^R_2 = \text{tan}^{-1}\left( \frac{r_{32}}{-r_{31}}\right) \\
        q^R_3 = \text{cos}^{-1}(\mathcal{R}_z^H \cdot \overrightarrow{p_{3e}})
    \end{gathered}
\end{equation}
The final joint angle is given by finding the angle between the human unit vector and the human forearm position.

\subsection{Low-level Control}
Due to noisiness in estimating human joint velocities, the desired robot arm joint velocities are set to zero, $\dot{q}^R_a = \mathbf{0}$. The computed desired joint positions are directly sent to the motors where the driver runs an onboard tracking PD controller at 40 MHz:
\begin{equation*}
    \tau_{com} = K_p (q - q_{des}) + K_d (\dot{q} - \dot{q}_{des}) + \tau_{ff}
\end{equation*}
where $\tau_{ff} = 0$. No gravity compensation is added as the design of the upper-body considers proximal actuation design principles \cite{YsimTellow}. This allows us to assume the arms are nearly massless. Furthermore, this design may also help ensure smooth robot arm movement in the absence of human joint velocity estimates. 

\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{Figures/HumanArmDiagram.pdf}
    \caption{The human arm motion is captured by the exoskeleton suit. Human joint angles are used to calculate the desired orientation of the robot elbow joint. The final stage involves approximating the robot shoulder as a spherical joint and solving for the desired joint angles.}
    \label{fig:arm_retargeting}
\end{figure}

==> SystemOverview.tex <==
\section{System Overview}
Keep this section short. Cite the previous system integram and Sunyu paper. Then discuss the upperbody of SATYRR and the joysticks. Mention new control rates, design philosophy for arms, etc.

The control architecture and layout were discussed in previous works \cite{Puru2022, wang2021dynamic}

Human motion can be used as a good kino-dynamic reference as it is highly stable in various environments and can generate large forces leveraging body dynamics and human balancing skills. We introduce a Human-Machine Interface (HMI) discussed in previous works \cite{Puru2022, wang2021dynamic} to capture the human motion. The human center of mass (CoM) and center of pressure (CoP) are captured by the linear actuators and force plate, respectively. The motion of two arms is measured by a passive motion capture system and kinematically mapped into the robot arm (Fig. xxxxxx).

==> raw_ideas.tex <==
\section{Motivation and Prior Work}
In previous papers we explored velocity control versus acceleration control for locomotion. We used heuristic mappings where the pitch of the human was filtered through  In this work we are trying to move towards whole-body teleoperation of highly dynamic movements. A simple heuristic approach to generating trajectories is to:

\begin{equation*}
    \begin{gathered}[b]
        \theta_R = \theta_H \\
        \dot{\theta_R} = \dot{\theta_H}
    \end{gathered}
\end{equation*}

This kinematic relationship cannot be satisfied (in theory) as the natural frequencies of the two pendulum like systems are inherently different:

\begin{equation*}
    \begin{gathered}
        \omega_R \neq \omega_H \\
        \dot{\theta_R} \neq \dot{\theta_H}
    \end{gathered}
\end{equation*}

Thus, we look at enforcing another kinematic similarity and try enforcing the DCM's of the two systems be the same. 
    
\section{Bilateral Teleoperation Derivation}

\subsection{Cart-Pole DCM}
We introduce bilateral teleoperation using dynamic similarity between a human LIP and robot cart-pole model. We use a cart-pole model to simplify the dynamics of the WIP.

\begin{figure}[h]
    \centering
    \includegraphics[width = \columnwidth]{Figures/CartPoleSketch.jpg}
    \caption{Cart Pole Model Sketch}
    \label{cartPoleSketch}
\end{figure}

The cart-pole dynamics are written as:

\begin{equation}
    \begin{gathered}[b] 
        (M+m)\ddot{x} - mLsin(\theta)\dot{\theta}^2 + mLcos(\theta)\ddot{\theta} = u(t)\\
        mL^2\ddot{\theta} + mLcos(\theta)\ddot{x} - mgLsin(\theta) = 0
    \end{gathered}
\end{equation}
using a small assumption $(sin(\theta) \approx \theta ; cos(\theta) \approx 1)$ and small pendulum velocities $(\dot{\theta}^2 \approx 0)$:

\begin{equation}\label{eqn:approximated_eq}
    \begin{gathered}[b]
        (M+m)\ddot{x} + mL\ddot{\theta} = u(t)\\
        mL^2\ddot{\theta} + mL\ddot{x} - mgL\theta = 0
    \end{gathered}
\end{equation}
solving for $\ddot{x}$ and $\ddot{\theta}$ we can rewrite as such:
\begin{equation}\label{eqn:rearranged_eq}
    \begin{gathered}[b] 
        \ddot{x} = \frac{u(t)}{M+m} - \frac{mL}{M+m}\ddot{\theta}\\
        \ddot{\theta} =  \frac{(M+m)g}{ML}\theta - \frac{u(t)}{ML}
    \end{gathered}
\end{equation}

\yeongtae{Inserting $\ddot{\theta}$ of (\ref{eqn:rearranged_eq}) into (\ref{eqn:approximated_eq}) yields:
\begin{equation}
\begin{gathered}
        \ddot{x} = \frac{m}{M}g\theta - \frac{u(t)}{m}\\
        \marty{\ddot{x} = \frac{u(t)}{M} - \frac{mg}{M}\theta}
\end{gathered}
\end{equation}
I think this equation is very important for cart-pole system since it describes horizontal dynamics. There is no horizontal motion if this equation is neglected and assuming zero initial horizontal velocity. Also, there is no way to justify $M >> m$ assumption for SATYRR. I updated the matrix ($0 \texttt{ ->  }\frac{m}{M}g$). Good news is it does not affect to the eigenvalues nor the isolation of $\theta$. However, it affects to the simulation. Please check your labview vi and correct the simulation codes.
}
\marty{I think this is a good point. I also think that the justification using the MFDCM concept to decouple the equations, as you mentioned below, does make this valid then.}

%Assuming that $M >> m$ we can rewrite in state space form:

\begin{equation} 
    \label{linStateSpaceModel}
    \begin{bmatrix}
        \dot{x}\\ \ddot{x}\\ \dot{\theta}\\ \ddot{\theta}
    \end{bmatrix} = 
    \begin{bmatrix}
        0 & 1 & 0 & 0\\
        0 & 0 & -\frac{m}{M}g & 0\\
        0 & 0 & 0 & 1\\
        0 & 0 & \frac{g}{L} & 0
    \end{bmatrix}
    \begin{bmatrix}
        x\\ \dot{x}\\ \theta\\ \dot{\theta}
    \end{bmatrix} +
    \begin{bmatrix}
        0 \\
        \frac{1}{M}\\
        0\\
        \frac{-1}{ML}
    \end{bmatrix} u(t)
\end{equation}
Looking at this system approximated at its fixed point, solving the characteristic equation and finding the eigenvalues we find:
\begin{equation}
    \begin{gathered}[b]
        \lambda_1 = \lambda_2 = 0 \\
        \lambda_3 = \sqrt{\frac{g}{L}}\\
        \lambda_4 = -\sqrt{\frac{g}{L}}
    \end{gathered}
\end{equation}
decoupling the $x$ and $\dot{x}$ terms,isolating the variables $\theta$ and $\dot{\theta}$ to focus on the unstable roots as to design control inputs that stabilize the system we can rewrite the equations above as:
\begin{equation}
    \begin{bmatrix}
        \dot{\theta}\\ \ddot{\theta}
    \end{bmatrix} = 
    \begin{bmatrix}
        0 & 1\\
        \omega^2 & 0
    \end{bmatrix}
    \begin{bmatrix}
        \theta\\ \dot{\theta}
    \end{bmatrix} +
    \begin{bmatrix}
        0 \\
        \frac{-1}{ML}
    \end{bmatrix} u(t)
\end{equation}
where $\omega = \sqrt{\frac{g}{L}}$. We notice immediately that decoupling terms to focus on the unstable roots our dynamics evolve similar to that of just an linear inverted pendulum. Note, however, that the control input matrix is different compared to that of the LIP.

Diagonlizing the matrix to isolate the convergent and divergent components of motion (DCM) we find the state transformation matrix $P$:

\begin{equation}
    P = \begin{bmatrix}
        1 & 1\\
        -\omega & \omega
    \end{bmatrix} 
\end{equation}


\begin{equation}
    \begin{bmatrix}
        \zeta \\ \xi
    \end{bmatrix} =
    P^{-1}q =
    \begin{bmatrix}
        \theta - \frac{\dot{\theta}}{\omega}\\
        \theta + \frac{\dot{\theta}}{\omega}
    \end{bmatrix}
\end{equation}
applying the transformation we can rewrite our equation as such:
 
\begin{equation}
    \begin{bmatrix}
        \dot{\zeta}\\ \dot{\xi}
    \end{bmatrix} = 
    \begin{bmatrix}
        -\omega & 0\\
        0 & \omega
    \end{bmatrix}
    \begin{bmatrix}
        \zeta\\ \xi
    \end{bmatrix} +
    \begin{bmatrix}
        \frac{1}{\omega ML} \\
        -\frac{1}{\omega ML}
    \end{bmatrix} u(t)
\end{equation}

Thus we clearly see that the cart-pole DCM, analogous to that of the LIP, is given by $\xi = \theta + \frac{\dot{\theta}}{\omega}$ and the DCM velocity in terms of the cart-pole dynamics is given by $\dot{\xi} = \omega \xi - \frac{u(t)}{\omega ML}$ 

\subsection{Straight to Dynamic Similarity}

We try to find a dynamic relationship between that of the human and that of the cart-pole system. What we ideally want is some sort of equality between the DCMs of the system:

\begin{equation}
    \begin{gathered}[b]
        \xi_R = \xi_H  \\
    \end{gathered}
\end{equation}
However the units do not match and what we really want is some type of non-dimensionless equality as such:
\begin{equation}
    \label{idealLaw}
    \theta_R + \frac{\dot{\theta_R}}{\omega_R} = \theta_H + \frac{\dot{\theta_H}}{\omega_H} 
\end{equation}

\yeongtae{Bottom of (\ref{idealLaw}) is MFDCM, not the original DCM.  We need to talk about MFDCM before introducing bottom of (\ref{idealLaw}).}

Either of these relationships are difficult to establish. The top part of Eq. \ref{idealLaw} does not maintain the correct unit equivalencies. The bottom part of Eq.\ref{idealLaw} requires that the angles of the robot and the human be the same in the absence of any angular velocity, when $\dot{\theta}_R = 0$ and $\dot{\theta}_H = 0$, which may be difficult to enforce as $\theta$ is underactuated. 

\yeongtae{I think using (12), which are MFDCM, can be achieved by applying LQR controller of the robot for $\theta_R$ and $\dot{\theta_R}$ letting the weightings of $Q$ matrix 1 and 1/$\omega_R$. This will optimize the MFDCM tracking with the controller. Try this with the simple feedback for human using human MFDCM and robot MFDCM difference that I told you.}



We see that we cannot set the pitch velocities of the two systems equal to each other as we are modeling the systems as pendulums and each system has its own unique natural frequency. What we desire is:
\begin{equation}
    \label{DCMgeometricsimilarity}
    \frac{\xi_H}{h_H} = \xi_R
\end{equation}

\begin{equation}
    \label{desiredLaw}
    \frac{\dot{\xi}_H}{\omega_H h_H} = \frac{\dot{\xi}_R}{\omega_R}
\end{equation}
where the LIP DCM is given by $\xi_H = x_H + \frac{\dot{x}_H}{\omega_H}$. 

\yeongtae{Actually, $x_H$ is the LIP pendulum position, not the COP or cart. Notations are messed up from here.}

We notice that both sides are dimensionless. Expanding the right hand side of Eq. \ref{desiredLaw} we see:

\begin{equation}
    \label{rightSideExpanded}
    \begin{gathered}[b]
        \dot{\xi}_R = \omega_R \xi_R - \frac{u_R}{\omega_R m_R h_R} \\
        \frac{\dot{\xi}_R}{\omega_R } = \theta_R + \frac{\dot{\theta}_R }{\omega_R} - \frac{u_R}{\omega_R^2 m_R h_R}\\
        \Rightarrow \frac{\dot{\xi}_H}{\omega_H h_H} = \theta_R + \frac{\dot{\theta}_R }{\omega_R} - \frac{u_R}{\omega_R^2 m_R h_R}
    \end{gathered}
\end{equation}
Expanding the left hand side of the LIP dynamics:

\begin{equation}
    \begin{gathered}
        \dot{\xi}_H = \dot{x}_H + \frac{\ddot{x}_H}{\omega_H}\\
        \frac{\dot{\xi}_H}{\omega_H h_H} = \frac{\dot{x}_H}{\omega_H h_H} + \frac{\ddot{x}_H}{\omega_H^2 h_H}
    \end{gathered}
\end{equation}
Replacing the humans acceleration with the summation of their applied force, $F_H$, and the feedback force $F_{fb}$:

\begin{equation}
        \frac{\dot{\xi}_H}{\omega_H h_H} = \frac{\dot{x}_H}{\omega_H h_H} + \frac{F_H + F_{fb}}{\omega_H^2 m_H h_H}
\end{equation}
Plugging this back into eq. \ref{rightSideExpanded}, the resulting equations becomes:
\begin{equation}
    \label{leftSideExpnaded}
    \frac{\dot{x}_H}{\omega_H h_H} + \frac{F_H}{\omega_H^2 m_H h_H} + \frac{F_{fb}}{\omega_H^2 m_H h_H} = \theta_R + \frac{\dot{\theta}_R }{\omega_R} - \frac{u_R}{\omega_R^2 m_R h_R}
\end{equation}
At this point we note that by linearizing the human LIP and assuming a constant location for the center of pressure we have the following relationships:
\yeongtae{This assumption makes the human just naturally fall down, as a fixed pivot inverted pendulum. Or, if you keep constant height assumption of LIP, x just keep accelerating and the acceleration is accelerated as x is increased. LIP model controls x by changing p, which is the control input for the system. However, this LIP model itself is denied by this assumption ($p_H=c$). It seems like too strong assumption.}

\yeongtae{I think it is better to introduce moving frame DCM concept, which makes the same result with (18), because the frame is attached at p. We could say that we are interested in $\theta$ dynamics, especially the convergence of $\theta$ that make the human and robot keep stand up, which can be observed from the moving frame. This can be applied for both LIP and cart pole system, justifying the isolation of $\theta$ dynamics from the cart pole dynamics in section A.}


\begin{equation}
    \begin{gathered}
        p_H =  c\\
        sin(\theta_H) \approx \theta_H = \frac{x_H - p_H}{h_H}\\
        \Rightarrow \dot{x}_H = \dot{\theta}_H h_H
    \end{gathered}
\end{equation}
Plugging this relationship back into eq. \ref{leftSideExpnaded} we find the following:

\begin{equation}
    \label{allExpnaded}
    \frac{\dot{\theta}_H}{\omega_H} + \frac{F_H}{\omega_H^2 m_H h_H} + \frac{F_{fb}}{\omega_H^2 m_H h_H} = \theta_R + \frac{\dot{\theta}_R }{\omega_R} - \frac{u_R}{\omega_R^2 m_R h_R}
\end{equation}
Isolating the variables in terms of the force applied on the cart and feedback force we find either one of two relationships, where option A is given by:

\begin{equation}
    \begin{gathered}
        F_{fb} = \omega_H^2 m_H h_H \left[\theta_R + \left(\frac{\dot{\theta}_R}{\omega_R} - \frac{\dot{\theta}_H}{\omega_H} \right) \right] \\
        u_R = F_{cart,ideal} = -\frac{\omega_R^2 m_R h_R}{\omega_H^2 m_H h_H}F_H
    \end{gathered}
\end{equation}
Option B is given by:
\begin{equation}
    \begin{gathered}
        F_{fb} = \omega_H^2 m_H h_H \left(\frac{\dot{\theta}_R}{\omega_R} - \frac{\dot{\theta}_H}{\omega_H} \right) \\
        u_R = F_{cart,ideal}= (\theta_R -\frac{F_H}{\omega_H^2 m_H h_H})\omega_R^2 m_R h_R
    \end{gathered}
\end{equation}

Option B simplifies to:

\begin{equation}
        \label{ff_force}
            u_R = F_{cart,ideal} = (\theta_R - \theta_H)\omega_R^2 m_R h_R
\end{equation}

There are a bunch of other options I tried, but the only one that seemed to work even remotely as well was setting the $F_{fb} = 0$ and incorporating all the dynamic similarity terms into the feedforward term $u_R$.

Option C is given by:

\begin{equation}
    \begin{gathered}
        u_R = \omega_R^2 m_R h_R \left((\frac{\dot{\theta}_R}{\omega_R} - \frac{\dot{\theta}_H}{\omega_H}) + (\theta_R -\frac{F_H}{\omega_H^2 m_H h_H})  \right)\\
        F_{fb} = 0
    \end{gathered}
\end{equation}

\subsection{Regulating Robot DCM Error Dynamics}
The key idea here gives the human control of the error dynamics rather than creating a 1 to 1 mapping between the two systems:

\begin{equation}
    \frac{\xi_H}{h_H} = (\xi_R - \xi_R^*)
\end{equation}
where the operational point DCM is a function of the external force applied:
\begin{equation}
    \begin{gathered}
        \xi_R^* = \theta_R^* + \frac{\dot{\theta}_R^*}{\omega_R} \\
        \dot{\theta}_R^* = 0 \\
        \xi_R^* = \theta_R^* = f(F_{ext})
    \end{gathered}
\end{equation}
Can we assume here that the operating point velocity is zero for linearization and DCM estimation

\subsection{External Forces and Feed-forward Moments}
Just like in Professor Ramos's work we scale the external force that the robot experience back to the human and vice versa:

\begin{equation}
    \begin{gathered}
        F_{ext,H} = \frac{m_H h_H \omega_H^2}{m_R h_R \omega_R^2}F_{ext,R}
    \end{gathered}
\end{equation}

There is also information that can be gained from using the CoP that we are disregarding in the process of assuming a fixed base. Going from a LIP model to a inverted pendulum, we believe that viewing the base as an actuator more accurately represents the ability of the pendulum to stay upright and captures the CoP dynamics. As such we feed-forward the scaled moment created along the human CoM:

\begin{figure}[h]
    \centering
    \includegraphics[width =80]{Figures/FFMoment.jpg}
    \caption{Spring attached to Human IP}
    \label{fig:Spring_IP}
\end{figure}

\begin{equation}
    \begin{gathered}
        M_{ff,H} = r_H \times F_x \\
        h_H F_x = M_{ff,H} \\
        M_{ff,R} = \frac{m_R h_R^2 \omega_R^2}{m_H h_H^2 \omega_H^2}M_{ff,H}
    \end{gathered}
\end{equation}

Converting this feed-forward moment along the CoM of the robot to a force and applying a feedforward torque:

\begin{equation}
    \tau_{ff.moment} = \frac{r_W}{h_R}M_{ff,R}
\end{equation}

\section{Experimentation and Setup}
\subsection{State Transformation}

Using option B for the feedback we perform a change of variables to track the unitless DCMs of the cart pole and LIP rather than the pitch and pitch velocities:

\begin{equation}
    \begin{gathered} 
        q_R = T_R q_C \\
        A_R = T_R A_C T_R^{-1}\\
        B_R = T_R B_C \\
        q_R = 
        \begin{bmatrix}
            x\\ \dot{x}\\ X_{com} \\ \zeta_R
        \end{bmatrix} = 
        \begin{bmatrix}
            1 & 0 & 0 & 0\\
            0 & 0 & 1 & 0\\
            1 & h_R & 0 & 0\\
            0 & 1 & 0 & \frac{1}{\omega_R}
        \end{bmatrix}
        \begin{bmatrix}
            x\\ \theta\\ \dot{x} \\ \dot{\theta}
        \end{bmatrix}
    \end{gathered}
\end{equation}
Note here that \textbf{tracking of the $\boldsymbol{X_{CoM}}$ position is not needed}. We can now develop an LQR controller to track the desired states. As we do not care about the tracking of the CoM, we set the gain for this term equal to zero. $K = [-100, -100, 0, 300]$

\subsection{Wheel pos. and vel. trajectory generation using $F_{cart,ideal}$}
\textbf{THESE DID NOT WORK}

The human input $F_H$ is mapped to a cart force as seen in eqn. \ref{ff_force}. This feedforward force is can be used to solve the cart-pole equations for a desired cart acceleration,$\ddot{x}_{des}$. There are two options for mapping the acceleration:

Method A uses the assumption that $M>>m$:
\begin{equation}
    \begin{gathered}
        u_R = F_{cart,ideal} = (\theta_R - \theta_H)\omega_R^2 m_R h_R \\
        \ddot{x}_{R}^{des} = \frac{F_{cart,ideal}}{M} = \frac{\omega_R^2 m_R h_R}{M}(\theta_R - \theta_H)\\
        = \frac{gm_R}{M}(\theta_R - \theta_H)
    \end{gathered}
\end{equation}
Method B without mass asumptions (using eqns. \ref{linStateSpaceModel}) shows:
\begin{equation}
    \begin{gathered}
        F_{cart,ideal} = (\theta_R - \theta_H)\omega_R^2 m_R h_R \\
        \ddot{x}_R^{des}= \frac{F_{cart,ideal} - mg\theta_R}{M}\\
        = \frac{(\theta_R - \theta_H)\omega_R^2 m_R h_R - m_Rg\theta_R}{M}\\
        = \frac{(\theta_R - \theta_H) m_Rg - m_Rg\theta_R}{M}\\
        \ddot{x}_R^{des} = -\frac{gm_R}{M}\theta_H
    \end{gathered}
\end{equation}
Integrating the acceleration we find the desired inputs for our LQR:
\begin{equation}
    \begin{gathered}
        \dot{x}_{des} = \int \ddot{x}_{des} dt\\
        x_{des} = \int \int \dot{x}_{des} dt dt
    \end{gathered}
\end{equation}

The error states and LQR are applied as such:
\begin{equation}
    \begin{gathered}
        f_{cart} = -K*\Bar{q}_R\\
        F_{cart} = -
        \begin{bmatrix}
        -100 & -100 & 0 & 300    
        \end{bmatrix}
        \begin{bmatrix}
            x-x_{des}\\ \dot{x} - \dot{x}_{des}\\ X_{com} - 0 \\ \xi_R - \frac{\xi_H}{h_H}
        \end{bmatrix}
    \end{gathered}
\end{equation}

The applied force on the cart-pole robot, added with step input disturbances is given by:
\begin{equation}
    F_{applied} = F_{cart} + F_D
\end{equation}
where $F_D \in [-50, 50]$ Newtons.

\subsection{Wheel pos. and vel. trajectory Generation with $F_{ff} = F_{cart,ideal}$}
Rather than generating a trajectory from the ideal cart force, we simply treat $F_{cart,ideal}$ as a feed-forward force and only track the DCM. With position and velocity tracking DCM tracking degrades as the robot is forced to choose between tracking the wheel position/velocity and the robot DCM. We find great DCM tracking and feedback with the following:

\begin{equation}
    \begin{gathered}
        F_{applied} = -K*\Bar{q}_R + F_{ff}\\
        F_{applied} = -
        \begin{bmatrix}
        0 & 0 & 0 & 300    
        \end{bmatrix}
        \begin{bmatrix}
            x-x_{des}\\ \dot{x} - \dot{x}_{des}\\ X_{com} - 0 \\ \xi_R - \frac{\xi_H}{h_H}
        \end{bmatrix} + F_{ff} \\
        = -300(\xi_R - \frac{\xi_H}{h_H}) + (\theta_R - \theta_H)\omega_R^2 m_R h_R 
    \end{gathered}
\end{equation}

Nonetheless, without wheel position and velocity tracking the robot can be difficult to control and drifts. To reduce this issues especially on hardware where oscillations are inevitable we can try to solve for a trajectory in steady state. 

\textbf{This does not work:}

Assuming in steady state $\ddot{\theta} = 0$ and from \ref{eqn:approximated_eq}:

\begin{equation}
\begin{gathered}
    mL^2\ddot{\theta_R} + mL\ddot{x_R} - mgL\theta_R = 0 \\
    \ddot{x}_{R}^{des} = g\theta_R
\end{gathered}
\end{equation}
Integrating we can find the desired wheel velocity and position. This strategy may work for locomotion but will fail when making contact with an environment. The desired positon and velocity terms will drift too far from the achievable ones causing the robot to slip.

\subsection{System with Spring}
Because the spring is intuitive to use and offers some benefits in terms of pilot control (reduces risk of falling over) we try to attach a spring to the original human pendulum model as seen below:
\begin{figure}[h]
    \centering
    \includegraphics[width =160]{Figures/SpringLIP.jpg}
    \caption{Spring attached to Human IP}
    \label{fig:Spring_IP}
\end{figure}

Writing down the net force equation we find that the spring effectively reduces the natural frequency of the pendulum. This makes sense as a free falling pendulum with a spring would fall slower:

\begin{equation}
    \begin{gathered}
        \ddot{x}_H = \omega_H^2(x_H - p)\\
        F_H + F_{spring} = F_{net} = m_H\omega_H^2(x_H - p) - K_s x_H\\
        =  m_H\omega_H^2 x_H - m_H K_{\omega} x_H \\
        = m_H(\omega_H^2 - K_{\omega}) x_H \\
        = m_H\omega_{new}^2 x_H
    \end{gathered}
\end{equation}
 Moreover, when working out the effect of the spring on the dynamic similarity terms we find a key issue. The reference term for the robot is effectively smaller:

 \begin{equation}
     \begin{gathered}
         u_R = \omega_R^2 m_R h_R(\theta_R - (\theta_H - \frac{K_{\omega}}{\omega_H^2}\theta_H))
     \end{gathered}
 \end{equation}
We can see from the equation above that the human reference angle is effectively reduced by a ratio of $\frac{K_{\omega}}{\omega_H^2}$. This is no good because I now have to lean further to command the same type of forward angle which causes me to once again fall over, negative the benefit gained from the spring. Albeit, when leaning off the box the spring was very helpful.

Without the inclusion of the spring's dynamics in the equations of motion I actually found it easier to control the robot. The mix betweent these ideas is the key somewhere. 

\subsection{Moving Frame DCM (MFDCM)}
Here we have the moving frame DCM concept introduced by Yeongtae:
\begin{figure}[h]
    \centering
    \includegraphics[width =\columnwidth]{Figures/MFDCM_MFDCM.PNG}
    \caption{MFDCM to MFDCM}
    \label{fig:MFDCM_MFDCM}
\end{figure}


